SkillForgeBench: Evaluating Agent Reliability Grounded in Agent Skill Specifications

Evaluating an agent's ability to strictly satisfy diverse and procedurally complex requirements is essential to determining its practical reliability. Conducting such an evaluation demands agentic tasks that reconcile broad domain coverage with deep procedural complexity. Existing paradigms face a fundamental trade-off: expert-curated benchmarks achieve procedural depth but suffer from domain diversity bottlenecks, whereas crowdsourced benchmarks span diverse scenarios but lack execution rigor. To resolve this tension, we present SkillForgeBench, which leverages agent skills as unifying execution blueprints across three co-designed stages: (1) Resource Preparation uses domain-balanced skills to guide artifact retrieval, establishing broad workflow coverage; (2) Skill-driven Task Synthesis employs skills as procedural anchors to partition artifact roles, synthesize naturalistic task instructions, and package sandboxed scenarios for deep procedural execution; and (3) Holistic Evaluation Design translates skill-embedded requirements into fine-grained completion and process rubrics to enable strict requirement-level scoring. Comprising 842 sandboxed tasks across five major professional domains, SkillForgeBench reveals a steep capability hierarchy among eight mainstream agents, led by Opus 4.8 ($40.9\%$ strict completion). Requiring all constrains satisfaction uncovers severe capability bottlenecks across all model tiers that remain masked under individual rubric pass rates ($70.0\%$ to $85.7\%$ vs. $12.6\%$ to $40.9\%$). Crucially, under the external guidance from skills, top-tier agents obtain larger gains than low-tier agents (i.e., $\Delta 19.2\%$ for Opus 4.8 vs. $\Delta 5.8\%$ for Haiku 4.5). Finally, agents satisfy process rubrics far less frequently than completion rubrics (under $3\%$ for Haiku 4.5), proving that completion-only checks overestimate real-world agent reliability.

==> sections/class_tables/BIZ.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\caption{
\textbf{Aligned masked scores for Business \& Finance under loose and strict credit.}
Task-level averages for completion with and without the skill, and for
instruction following with the skill, evaluated on the aligned task set.
Under \textit{loose} credit a task earns the mean score of its criteria;
under \textit{strict} credit it earns full credit only when \emph{every}
criterion attains its maximum score, and zero otherwise.
Average total, tool-call, and agent-thought step counts are reported for
with-skill and no-skill runs. Total steps equal tool-call steps plus
agent-thought steps plus two.
\textbf{Bold} marks the best score in each score column.
}
\label{tab:aligned_raw_scores_biz}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l rrr rrr p{6pt} rr rr rr@{}}
\toprule
& \multicolumn{3}{c}{\cellcolor{aegisgreen}\textcolor{white}{\textbf{Loose}}}
& \multicolumn{3}{c}{\cellcolor{aegisgreen!80!black}\textcolor{white}{\textbf{Strict}}}
& {}
& \multicolumn{6}{c}{\cellcolor{aegisgreen!60!black}\textcolor{white}{\textbf{Efficiency}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){9-14}
\textbf{Model}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& {}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Total steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Tool-call steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Agent-thought steps}} \\
\cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& {}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill \\
\midrule
\rowcolor{aegiszebra}
Opus 4.8 & \textbf{92.7} & \textbf{83.4} & \textbf{91.7} & 51.2 & \textbf{28.0} & 37.9 & {} & 63.3 & 55.1 & 36.1 & 31.9 & 25.1 & 21.2 \\
GLM-5.2 & 91.7 & 81.5 & 91.6 & \textbf{55.0} & 25.6 & \textbf{39.8} & {} & 82.0 & 72.5 & 46.1 & 40.4 & 33.9 & 30.1 \\
\rowcolor{aegiszebra}
HY3 & 87.8 & 75.9 & 90.1 & 35.5 & 12.3 & 30.3 & {} & 66.9 & 57.0 & 36.3 & 30.6 & 28.6 & 24.4 \\
Sonnet 4.6 & 89.1 & 80.2 & 83.0 & 45.0 & 20.4 & 14.2 & {} & 40.9 & 32.4 & 28.4 & 22.5 & 10.6 & 7.92 \\
\rowcolor{aegiszebra}
Haiku 4.5 & 79.0 & 70.3 & 66.6 & 15.2 & 9.00 & 2.37 & {} & 48.8 & 40.7 & 24.6 & 21.1 & 22.2 & 17.6 \\
Kimi K2.6 & 85.7 & 75.0 & 78.8 & 28.9 & 14.2 & 9.00 & {} & 58.2 & 51.3 & 32.2 & 27.3 & 24.0 & 22.0 \\
\rowcolor{aegiszebra}
Qwen3.5-397B-A17B & 80.2 & 71.0 & 69.0 & 21.3 & 4.74 & 3.79 & {} & 40.4 & 33.1 & 27.3 & 22.1 & 11.1 & 9.01 \\
Gemini 3.6 Flash & 82.0 & 74.0 & 74.8 & 22.3 & 8.53 & 5.21 & {} & 71.8 & 66.0 & 34.7 & 31.7 & 35.1 & 32.3 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> sections/class_tables/CREATIVE.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\caption{
\textbf{Aligned masked scores for Creative under loose and strict credit.}
Task-level averages for completion with and without the skill, and for
instruction following with the skill, evaluated on the aligned task set.
Under \textit{loose} credit a task earns the mean score of its criteria;
under \textit{strict} credit it earns full credit only when \emph{every}
criterion attains its maximum score, and zero otherwise.
Average total, tool-call, and agent-thought step counts are reported for
with-skill and no-skill runs. Total steps equal tool-call steps plus
agent-thought steps plus two.
\textbf{Bold} marks the best score in each score column.
}
\label{tab:aligned_raw_scores_creative}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l rrr rrr p{6pt} rr rr rr@{}}
\toprule
& \multicolumn{3}{c}{\cellcolor{aegisgreen}\textcolor{white}{\textbf{Loose}}}
& \multicolumn{3}{c}{\cellcolor{aegisgreen!80!black}\textcolor{white}{\textbf{Strict}}}
& {}
& \multicolumn{6}{c}{\cellcolor{aegisgreen!60!black}\textcolor{white}{\textbf{Efficiency}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){9-14}
\textbf{Model}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& {}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Total steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Tool-call steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Agent-thought steps}} \\
\cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& {}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill \\
\midrule
\rowcolor{aegiszebra}
Opus 4.8 & \textbf{86.3} & \textbf{80.6} & \textbf{86.3} & \textbf{44.1} & \textbf{25.0} & \textbf{27.9} & {} & 68.8 & 62.8 & 39.9 & 37.0 & 26.9 & 23.8 \\
GLM-5.2 & 84.9 & 78.0 & 84.3 & 42.6 & 21.3 & 27.2 & {} & 98.7 & 97.1 & 56.4 & 55.6 & 40.3 & 39.4 \\
\rowcolor{aegiszebra}
HY3 & 81.1 & 73.5 & 82.7 & 30.9 & 15.4 & 17.6 & {} & 72.6 & 64.7 & 39.7 & 35.7 & 30.9 & 27.1 \\
Sonnet 4.6 & 82.3 & 74.9 & 76.9 & 30.1 & 15.4 & 9.56 & {} & 57.0 & 43.6 & 39.3 & 29.5 & 15.7 & 12.1 \\
\rowcolor{aegiszebra}
Haiku 4.5 & 70.3 & 63.5 & 63.4 & 15.4 & 6.62 & 3.68 & {} & 57.9 & 47.1 & 30.3 & 25.4 & 25.6 & 19.7 \\
Kimi K2.6 & 77.7 & 71.9 & 70.4 & 21.3 & 11.0 & 2.94 & {} & 75.7 & 69.7 & 41.8 & 38.1 & 31.9 & 29.6 \\
\rowcolor{aegiszebra}
Qwen3.5-397B-A17B & 71.6 & 65.4 & 60.4 & 11.8 & 6.62 & 1.47 & {} & 48.3 & 42.3 & 32.5 & 28.1 & 13.8 & 12.2 \\
Gemini 3.6 Flash & 79.8 & 73.0 & 70.5 & 16.9 & 8.82 & 2.94 & {} & 91.6 & 80.4 & 45.0 & 39.1 & 44.7 & 39.3 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> sections/class_tables/HARNESS_BEHAVIOR.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\caption{
\textbf{Aligned masked scores for Harness Behavior under loose and strict credit.}
Task-level averages for completion with and without the skill, and for
instruction following with the skill, evaluated on the aligned task set.
Under \textit{loose} credit a task earns the mean score of its criteria;
under \textit{strict} credit it earns full credit only when \emph{every}
criterion attains its maximum score, and zero otherwise.
Average total, tool-call, and agent-thought step counts are reported for
with-skill and no-skill runs. Total steps equal tool-call steps plus
agent-thought steps plus two.
\textbf{Bold} marks the best score in each score column.
}
\label{tab:aligned_raw_scores_harness_behavior}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l rrr rrr p{6pt} rr rr rr@{}}
\toprule
& \multicolumn{3}{c}{\cellcolor{aegisgreen}\textcolor{white}{\textbf{Loose}}}
& \multicolumn{3}{c}{\cellcolor{aegisgreen!80!black}\textcolor{white}{\textbf{Strict}}}
& {}
& \multicolumn{6}{c}{\cellcolor{aegisgreen!60!black}\textcolor{white}{\textbf{Efficiency}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){9-14}
\textbf{Model}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& {}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Total steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Tool-call steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Agent-thought steps}} \\
\cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& {}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill \\
\midrule
\rowcolor{aegiszebra}
Opus 4.8 & \textbf{82.8} & \textbf{74.4} & \textbf{87.2} & \textbf{32.5} & 11.9 & 23.0 & {} & 74.0 & 65.3 & 42.2 & 38.8 & 29.8 & 24.5 \\
GLM-5.2 & 80.9 & 72.7 & 82.6 & 25.4 & \textbf{13.5} & \textbf{25.4} & {} & 109 & 101 & 60.9 & 56.7 & 46.1 & 41.8 \\
\rowcolor{aegiszebra}
HY3 & 78.5 & 73.7 & 83.7 & 19.8 & 11.9 & 19.8 & {} & 82.9 & 78.7 & 44.6 & 43.1 & 36.3 & 33.6 \\
Sonnet 4.6 & 78.3 & 68.2 & 76.6 & 15.9 & 4.76 & 9.52 & {} & 62.9 & 48.0 & 42.9 & 33.2 & 18.0 & 12.8 \\
\rowcolor{aegiszebra}
Haiku 4.5 & 64.3 & 58.4 & 64.6 & 7.94 & 2.38 & 1.59 & {} & 72.0 & 62.7 & 37.9 & 33.4 & 32.1 & 27.2 \\
Kimi K2.6 & 73.1 & 69.1 & 74.0 & 10.3 & 5.56 & 7.14 & {} & 95.9 & 81.1 & 51.6 & 42.5 & 42.4 & 36.6 \\
\rowcolor{aegiszebra}
Qwen3.5-397B-A17B & 67.9 & 64.8 & 66.4 & 9.52 & 2.38 & 3.97 & {} & 63.4 & 55.0 & 41.4 & 34.7 & 20.0 & 18.2 \\
Gemini 3.6 Flash & 78.8 & 66.8 & 70.5 & 18.3 & 2.38 & 11.1 & {} & 106 & 97.5 & 52.4 & 48.0 & 51.8 & 47.5 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> sections/class_tables/KNOWLEDGE.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\caption{
\textbf{Aligned masked scores for Knowledge under loose and strict credit.}
Task-level averages for completion with and without the skill, and for
instruction following with the skill, evaluated on the aligned task set.
Under \textit{loose} credit a task earns the mean score of its criteria;
under \textit{strict} credit it earns full credit only when \emph{every}
criterion attains its maximum score, and zero otherwise.
Average total, tool-call, and agent-thought step counts are reported for
with-skill and no-skill runs. Total steps equal tool-call steps plus
agent-thought steps plus two.
\textbf{Bold} marks the best score in each score column.
}
\label{tab:aligned_raw_scores_knowledge}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l rrr rrr p{6pt} rr rr rr@{}}
\toprule
& \multicolumn{3}{c}{\cellcolor{aegisgreen}\textcolor{white}{\textbf{Loose}}}
& \multicolumn{3}{c}{\cellcolor{aegisgreen!80!black}\textcolor{white}{\textbf{Strict}}}
& {}
& \multicolumn{6}{c}{\cellcolor{aegisgreen!60!black}\textcolor{white}{\textbf{Efficiency}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){9-14}
\textbf{Model}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& {}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Total steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Tool-call steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Agent-thought steps}} \\
\cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& {}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill \\
\midrule
\rowcolor{aegiszebra}
Opus 4.8 & \textbf{93.7} & \textbf{86.5} & 89.8 & \textbf{62.8} & \textbf{32.7} & 31.9 & {} & 69.1 & 63.9 & 39.9 & 37.8 & 27.2 & 24.2 \\
GLM-5.2 & 89.5 & 83.0 & \textbf{90.7} & 47.8 & 25.7 & \textbf{42.5} & {} & 99.0 & 91.6 & 55.6 & 52.2 & 41.3 & 37.4 \\
\rowcolor{aegiszebra}
HY3 & 87.7 & 80.9 & 84.7 & 45.1 & 20.4 & 24.8 & {} & 74.7 & 72.2 & 41.0 & 39.2 & 31.7 & 31.0 \\
Sonnet 4.6 & 90.5 & 83.0 & 79.6 & 42.5 & 23.9 & 10.6 & {} & 51.6 & 39.1 & 36.3 & 27.3 & 13.3 & 9.79 \\
\rowcolor{aegiszebra}
Haiku 4.5 & 79.0 & 73.5 & 66.2 & 15.9 & 10.6 & 0.885 & {} & 54.1 & 46.5 & 27.4 & 24.2 & 24.7 & 20.3 \\
Kimi K2.6 & 85.2 & 80.9 & 74.6 & 31.0 & 16.8 & 6.19 & {} & 71.0 & 65.8 & 39.0 & 33.9 & 30.0 & 29.9 \\
\rowcolor{aegiszebra}
Qwen3.5-397B-A17B & 79.0 & 74.4 & 68.5 & 18.6 & 5.31 & 2.65 & {} & 43.1 & 36.7 & 29.1 & 23.9 & 11.9 & 10.7 \\
Gemini 3.6 Flash & 86.0 & 79.7 & 73.7 & 31.9 & 19.5 & 4.42 & {} & 85.8 & 86.4 & 42.0 & 42.0 & 41.8 & 42.4 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> sections/class_tables/TECH.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\caption{
\textbf{Aligned masked scores for Technology \& Engineering under loose and strict credit.}
Task-level averages for completion with and without the skill, and for
instruction following with the skill, evaluated on the aligned task set.
Under \textit{loose} credit a task earns the mean score of its criteria;
under \textit{strict} credit it earns full credit only when \emph{every}
criterion attains its maximum score, and zero otherwise.
Average total, tool-call, and agent-thought step counts are reported for
with-skill and no-skill runs. Total steps equal tool-call steps plus
agent-thought steps plus two.
\textbf{Bold} marks the best score in each score column.
}
\label{tab:aligned_raw_scores_tech}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l rrr rrr p{6pt} rr rr rr@{}}
\toprule
& \multicolumn{3}{c}{\cellcolor{aegisgreen}\textcolor{white}{\textbf{Loose}}}
& \multicolumn{3}{c}{\cellcolor{aegisgreen!80!black}\textcolor{white}{\textbf{Strict}}}
& {}
& \multicolumn{6}{c}{\cellcolor{aegisgreen!60!black}\textcolor{white}{\textbf{Efficiency}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){9-14}
\textbf{Model}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Compl.}
& \cellcolor{aegislight}\footnotesize\textbf{Follow.}
& {}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Total steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Tool-call steps}}
& \multicolumn{2}{c}{\cellcolor{aegislight}\footnotesize\textbf{Agent-thought steps}} \\
\cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& {}
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill
& \cellcolor{aegislight}\footnotesize w/ skill
& \cellcolor{aegislight}\footnotesize wo/ skill \\
\midrule
\rowcolor{aegiszebra}
Opus 4.8 & \textbf{77.4} & \textbf{75.6} & \textbf{84.9} & \textbf{24.9} & 14.8 & \textbf{19.5} & {} & 79.6 & 75.0 & 45.4 & 44.9 & 32.2 & 28.0 \\
GLM-5.2 & 76.4 & 71.5 & 84.1 & 19.5 & \textbf{15.2} & 16.0 & {} & 120 & 115 & 68.1 & 66.1 & 49.8 & 47.1 \\
\rowcolor{aegiszebra}
HY3 & 73.0 & 69.0 & 80.0 & 14.4 & 12.8 & 16.0 & {} & 98.8 & 93.8 & 54.5 & 52.1 & 42.3 & 39.6 \\
Sonnet 4.6 & 72.5 & 71.4 & 68.0 & 14.0 & 11.3 & 7.39 & {} & 65.4 & 51.6 & 44.1 & 34.6 & 19.3 & 15.0 \\
\rowcolor{aegiszebra}
Haiku 4.5 & 61.2 & 58.2 & 57.6 & 9.73 & 5.45 & 2.72 & {} & 76.9 & 68.5 & 40.9 & 37.2 & 34.0 & 29.3 \\
Kimi K2.6 & 70.9 & 67.6 & 68.2 & 12.1 & 8.95 & 4.67 & {} & 103 & 93.8 & 55.3 & 49.8 & 46.0 & 42.0 \\
\rowcolor{aegiszebra}
Qwen3.5-397B-A17B & 63.4 & 60.8 & 58.5 & 7.00 & 6.61 & 1.56 & {} & 64.0 & 62.5 & 41.9 & 39.0 & 20.1 & 21.5 \\
Gemini 3.6 Flash & 73.5 & 68.0 & 66.8 & 10.1 & 7.78 & 3.50 & {} & 119 & 116 & 59.4 & 57.7 & 57.8 & 56.7 \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> sections/pending_constraint_finding.tex <==
% ============================================================================
% PENDING (not \input anywhere): the finding
%   "satisfying all constraints remains challenging and sharply separates agents"
% and the sentences that support it. These were taken out of the paper and the
% original sentences were restored in place. Each block names where it would go
% and which original sentence it would replace.
% ============================================================================

% --- iclr2027_conference.tex, abstract ---
% Would replace: "Evaluating eight state-of-the-art LLMs demonstrates that \textsc{SkillForgeBench} effectively discriminates model capability tiers, ..."
Evaluating eight state-of-the-art LLMs shows that satisfying all constraints remains challenging: even the leading agent, \textsc{Opus 4.8}, satisfies all constraints on the final outcome in only $40.9\%$ of tasks.

% --- iclr2027_conference.tex, abstract ---
% Would replace: "By enforcing strict rubric compliance, our evaluation scheme effectively uncovers brittle agent behaviors, ..."
Although agents pass most individual rubrics, requiring all constraints to hold simultaneously amplifies the gap between the strongest and weakest agents from $1.2\times$ under loose scoring to $3.2\times$ under strict scoring.

% --- sections/introduction.tex, last paragraph, second sentence ---
% Would replace: "The resulting leaderboard reveals a steep capability hierarchy: ..."
The resulting leaderboard shows that satisfying all constraints remains challenging and sharply separates agents: \textsc{Opus 4.8} leads at only $40.9\%$ strict completion, while \textsc{Qwen3.5-397B} and \textsc{Haiku 4.5} bottom out near $13\%$.

% --- sections/introduction.tex, last paragraph, first insight ---
% Would replace two sentences: "Crucially, strict evaluation reveals that ..." and "First, strict rubric compliance isolates ..."
First, agents satisfy most individual constraints but often fail to satisfy all of them: high individual rubric pass rates ($70.0\%$--$85.7\%$) give a false sense of capability, and requiring all constraints to hold simultaneously widens the gap between the strongest and weakest agents from $1.2\times$ to $3.2\times$.

% --- sections/conclusion.tex, finding (1) ---
% Would replace: "(1) strict, holistic constraint satisfaction defines the true capability divide between model tiers;"
(1) satisfying all constraints simultaneously, rather than individual constraints, defines the true capability divide between agents;

% --- sections/experiment.tex, Main Leaderboard paragraph ---
% Would replace the paragraph "Table~\ref{main_leaderboard_table} presents performance ...".
% Differences from the original: the "i.e., ..." clause, "only", the tier-definition sentence, and "separating into distinct groups".
Table~\ref{main_leaderboard_table} presents performance and trajectory efficiency across 8 frontier models evaluated with and without agent skill. \skillforgebench{} induces substantially long execution horizons: across models, with-skill runs require 15.5--47.0 total steps and 32.9--58.0 tool calls per task on average. Under the primary metric of \textit{strict-scoring completion with skill}, i.e., the proportion of tasks on which all constraints on the final outcome are satisfied, \textbf{Opus 4.8} leads the panel at only $40.9\%$, followed by \textbf{GLM-5.2} at $36.8\%$, with \textbf{Sonnet 4.6} and \textbf{HY3} tied at roughly $28\%$. Accordingly, we refer to Opus 4.8 and GLM-5.2 as top-tier agents, Sonnet 4.6 and HY3 as mid-tier agents, and the remaining four agents as lower-tier agents. Open-weight and proprietary models interleave throughout the ranking rather than separating into distinct groups.

% --- sections/experiment.tex, "Holistic Constraint Satisfaction Reveals Hidden Capability Gaps" paragraph ---
% Would replace the paragraph "While loose scoring evaluation suggests ...".
While loose scoring suggests a deceptively narrow gap in satisfying individual constraints (Haiku 4.5-$70.0\%$ to Opus 4.8-$85.7\%$, $1.2\times$), strict evaluation isolates holistic constraint satisfaction as the primary factor dividing model tiers, expanding the performance spread dramatically (Haiku 4.5-$12.6\%$ to Opus 4.8-$40.9\%$, $3.2\times$). Lower-tier agents routinely succeed on isolated rubrics but fail far more often when all constraints must hold simultaneously. Thus, the true gap between model tiers lies in satisfying all constraints simultaneously, not in isolation. This suggests shifting agent optimization from incremental rubric fixes to holistic constraint alignment.


==> sections/zhengxi_intro.tex <==
\section{Proposed Revision}

As language-model agents take on increasingly complex professional work~\citep{merrill2026terminalbenchbenchmarkingagentshard,ye2026clawevaltrustworthyevaluationautonomous}, establishing rigorous benchmarks to evaluate their real-world reliability has become essential.
In practical deployments, a reliable agent must not merely produce a superficially plausible final deliverable; it must strictly satisfy all the \textit{constraints} in human instructions, which specify {what agents must do}--\textit{obligation}--and {what agents must not do}--\textit{prohibition}--in outcomes and execution.
% The expectations to them are no longer only to produce outcomes that can work but also to satisfy detailed \textit{constraints} in human instructions, which specify {what agents must do}--\textit{obligation}--and {what agents must not do}--\textit{prohibition}--in outcomes and execution.
Failing to satisfy these constraints forces human users to intervene or re-issue instructions, defeating the practical utility of autonomous agents.
% At the same time, an important feature of truly helpful agents is their ability to satisfy all the constraints; otherwise, human users need to repeat the same constraints in the next prompt.
% Together, the new requirement for agents is to jointly satisfy all obligations and respect all prohibitions specified in human instructions.
% To assess agents performance, there is a need for benchmarks whose tasks contain multiple constraints and corresponding evaluation methods that truly reflect human needs in reality.

However, existing agentic benchmarks struggle to evaluate this multi-faceted reliability due to a fundamental dilemma in task curation.
Expert-curated benchmarks tasks contain carefully design constraints that truly reflect human needs, ensuring task realism, yet they remain strictly bottlenecked by manual authoring costs and confined to narrow domains~\citep{yang2026makes,DBLP:journals/corr/abs-2602-01244}.
Crowd-sourced and synthetic benchmarks achieve domain diversity, but the synthesis of task constraints usually do not reflect deep understanding to real-world human demands, ultimately yielding tasks drifted from practical importance~\citep{hua2026cliuniverse,han2026ridewaybenchmarkingefficienttask}.

Existing benchmarks towards this goal have been created in two primary paradigms and have two different properties.
(1) In \textbf{Expert-driven curation}, human experts design and write the constraints and graders within specialized domains, offering essential task \textbf{realism};
yet, it is strictly bottlenecked by manual authoring costs and cannot scale across diverse domains.
(2) In \textbf{Synthesis-driven curation}, LLMs generate constraints and graders from seed materials such as taxonomies or system prompts, offering domain \textbf{diversity};
yet, the synthesized constraints tend to lack realism,  e.g., imposing requirements
that real users rarely specify, since they are not grounded in actual user needs.
Consequently, neither paradigm yields benchmarks that simultaneously contain realistic and diverse constraints that humans impose in practice.

To bridge this gap, we leverage \textbf{Skills}, the native structural primitive in the agent ecosystem, as structured blueprints for execution-grounded benchmark synthesis.
Written by human experts, skills encode complex workflows, including explicit execution steps, domain-specific knowledge, and working conventions.
All of this information can be transformed into constraints that reflect human needs in \textbf{realistic} working scenarios.
Furthermore, the broad distribution of skills on the Internet guaranties domain \textbf{diversity}.

Building on this insight, we introduce \textsc{SkillForgeBench}, an agentic evaluation benchmark built on a skill-centric task synthesis pipeline.
Specifically, a skill serves as a synthesis blueprint to construct an agentic task.
First, in \textbf{resource preparation}, we curate a set of high-quality, domain-balanced skills, for each of which we search realistic (1) artifacts and (2) user queries on the Internet as two necessary components of an agentic task---an environment and an instruction.
Second, in \textbf{skill-driven task synthesis}, we transform the detailed workflow in the skill into constraints in the user instruction, which specify every detailed requirement of the task.
Third, in \textbf{contrastive rubric construction}, we compose evaluation rubrics with respect to constraints through contrasting the differences between two separate agent rollouts: one runs without skill and hence will not satisfy any constraints; another runs with skill and will satisfy the constraints; in addition, we introduce a \emph{strict} scoring regime that rewards agents only when they meet all the constraints.
In total, \textsc{SkillForgeBench} currently comprises 842 rigorously verified, sandboxed tasks across diverse domains, establishing a scalable testbed for agent capabilities to satisfy realistic constraints in human instruction.

We evaluate eight state-of-the-art LLM agents on \skillforgebench{}, covering leading proprietary and open-weight models on the same harness.
The resulting leaderboard reveals a steep capability hierarchy: top-performing frontier systems (led by \textsc{Opus 4.8} at $40.9\%$ strict completion) outpace mid-tier and weaker agents (e.g., \textsc{Qwen3.5-397B} and \textsc{Haiku 4.5}) by a wide margin, with the latter bottoming out near $12.6\%$.
Crucially, strict evaluation reveals that high individual rubric pass rates ($70.0\%$--$85.7\%$) give a false sense of capability, whereas requiring all constraints to hold simultaneously exposes severe execution bottlenecks across model tiers.
Beyond leaderboard rankings, trajectory-level diagnostic analyses yield three core insights: First, strict rubric compliance isolates true execution boundaries, showing that loose checks mask hidden trajectory failures. Second, explicit skills amplify existing reasoning rather than fixing missing capabilities, nearly doubling strict completion for top-performing models ($\Delta 19.2\%$ for \textsc{Opus 4.8}) while offering minimal gain to other systems ($\Delta 5.8\%$ for \textsc{Haiku 4.5}). Third, process auditing exposes frequent operational shortcuts, where baseline models skip verification loops to force partial deliverables, causing strict process scores for models like \textsc{Qwen3.5-397B} and \textsc{Haiku 4.5} to drop below $3\%$.

